Reject option models comprising out-of-distribution detection

The optimal prediction strategy for out-of-distribution (OOD) setups is a fundamental question in machine learning. In this paper, we address this question and present several contributions. We propose three reject option models for OOD setups: the Cost-based model, the Bounded TPR-FPR model, and the Bounded Precision-Recall model. These models extend the standard reject option models used in non-OOD setups and define the notion of an optimal OOD selective classifier. We establish that all the proposed models, despite their different formulations, share a common class of optimal strategies. Motivated by the optimal strategy, we introduce double-score OOD methods that leverage uncertainty scores from two chosen OOD detectors: one focused on OOD/ID discrimination and the other on misclassification detection. The experimental results consistently demonstrate the superior performance of this simple strategy compared to state-of-the-art methods. Additionally, we propose novel evaluation metrics derived from the definition of the optimal strategy under the proposed OOD rejection models. These new metrics provide a comprehensive and reliable assessment of OOD methods without the deficiencies observed in existing evaluation approaches.

==> sandbox.tex <==
\section{Reject option models: non-OOD setup}

Let $\SX$ be the set of observations. Let $\SY$ be a finite set of labels. Let $p_I\colon\SX\times\SY\rightarrow\Re_+$ be a joint distribution of observations and labels. The goal in the non-reject setting is to find a classifier $h\colon\SX\rightarrow\SY$ with a small expected risk
\[ R(h) = \int_{\SX} \sum_{y\in\SY} \ell(y,h(x))\,dx
\]
%
where $\ell \colon \SY\times\SY\rightarrow\Re_+$ is a loss penalizing the predictions. The expected risk can be reduced by abstaining from prediction in uncertain cases. To this end, we use a selective classifier $(h,c)$ composed of a classifier $h\colon\SX\rightarrow\SY$ and a selection function $c\colon\SX\rightarrow[0, 1]$. When applying the selective classifier to input $x\in\SX$ it outputs 
\[
   (h,c)(x) = \left \{ \begin{array}{rcl}
     h(x) & \mbox{with probability} & c(x) \\
     \mbox{reject} & \mbox{reject with probability} & 1-c(x)\\
    \end{array}
    \right .
\]

\subsection{Cost-based model}
Besides the label loss $\ell\colon\SY\times\SY\rightarrow\Re_+$, let us define a reject loss $\veps \in\Re_+$ incurred when a classifier rejects to predict. The selective classifier $(h,c)$ is then evaluated in terms of the expected risk 
%\[
 \begin{equation}
 \label{equ:NonOODCostBasedRisk}
  R_B(h,c) \! = \!\! \int_{\SX} \! \sum_{y\in\SY} p_I(x,y)\,\big (\ell(y,h(x)) c(x)
   + (1-c(x))\veps\big ) dx\:.
\end{equation}
%\]

\begin{definition}[Cost-based model]\label{def:nonOODCostBased} The optimal selective classifier $(h_B,c_B)$ is a solution to the minimization problem
%
\begin{equation}
   \min_{h,c} R_B(h,c)  \,,
\end{equation}
%
where we assume that both minimizers exist. 
\end{definition}
The well-known optimal strategy $(h_B,c_B)$ of the cost-based model given in Definition~\ref{def:nonOODCostBased} reads
\begin{eqnarray}
  \label{equ:bayesPredictor}
   h_B(x) \in \argmin_{\hat{y}\in\SY} \sum_{y\in\SY} p(y\mid x) \,
   \ell(y,\hat{y}) \:,  \\
  \label{equ:BayesOptimalRejection}
   c_B(x) = \left \{ \begin{array}{rcl}
       1 & \mbox{if} & r^*(x) < \veps \:, \\
       \tau& \mbox{if} & r^*(x) = \veps  \:, \\
       0 & \mbox{if} & r^*(x) > \veps \:,\       
     \end{array} \right .
\end{eqnarray}
%
where 
\[
   r^*(x) = \min_{\hat{y}\in\SY} \sum_{y\in\SY} p(y\mid x) \, \ell(y,\hat{y})
\] 
%
is the minimal conditional expected risk associated with input $x$, and 
% and a selection function 
%\begin{equation}
%  \label{equ:BayesOptimalRejection}
%   c_B(x) = \left \{ \begin{array}{rcl}
%       1 & \mbox{if} & r^*(x) < \veps \:, \\
%       0 & \mbox{if} & r^*(x) > \veps \:, \\       
%       \tau& \mbox{if} & r^*(x) = \veps \:. \       
%     \end{array} \right .
%\end{equation}
$\tau$ is any real number from the interval $[0,1]$. In the boundary case when $r^*(x)=\veps$ one can arbitrarily reject or return the best label $h_B(x)$ without affecting the value of the risk $R_B(h,c)$. In turn, there always exists a deterministic optimal strategy solving the cost-based model. In the sequel, we denote the classifier $h_B$ alone as {\em Bayes classifier}.

